High-mass star-forming cloud G0.38+0.04 in the Galactic Center Dust Ridge contains H2CO and SiO masers

We have discovered a new H$_2$CO (formaldehyde) $1_{1,0}-1_{1,1}$ 4.82966 GHz maser in Galactic Center Cloud C, G0.38+0.04. At the time of acceptance, this is the eighth region containing an H$_2$CO maser detected in the Galaxy. Cloud C is one of only two sites of confirmed high-mass star formation along the Galactic Center Ridge, affirming that H$_2$CO masers are exclusively associated with high-mass star formation. This discovery led us to search for other masers, among which we found new SiO vibrationally excited masers, making this the fourth star-forming region in the Galaxy to exhibit SiO maser emission. Cloud C is also a known source of CH$_3$OH Class-II and OH maser emission. There are now two known SiO and H$_2$CO maser containing regions in the CMZ, compared to two and six respectively in the Galactic disk, while there is a relative dearth of H$_2$O and CH$_3$OH Class-II masers in the CMZ. SiO and H$_2$CO masers may be preferentially excited in the CMZ, perhaps due to higher gas-phase abundances from grain destruction and heating, or alternatively H$_2$O and CH$_3$OH maser formation may be suppressed in the CMZ. In any case, Cloud C is a new testing ground for understanding maser excitation conditions.

==> aamacros.tex <==
\newcommand\arcdeg{\mbox{$^\circ$}\xspace}
